Majority Kernels: An Approach to Leverage Big Model Dynamics for Efficient Small Model Training

Recent breakthroughs and successful deployment of large language and vision models in a constrained environment predominantly follow a two phase approach. First, large models are trained to achieve peak performance, followed by a model shrinking method to meet hardware constraints; Methods like distillation, compression or quantization help leverage the highly performant large models to induce smaller performant ones. Formally, this can be seen as the problem of identifying an optimal model of size $n$ from a larger model of size $k \cdot n$, where $k > 1$ is the overparameterization factor. This paper explores the hypothesis that a single training run can simultaneously train a larger model for performance and derive a smaller model for deployment. Our contribution is an effective architectural change, namely, {\it Majority Kernels} that is compatible with the main standard architectures such as multi-layer perceptrons (MLPs), Residual networks (ResNets), and Transformers. We demonstrate that applying our technique can modify the training dynamics resulting in performance gains across architectures and tasks while maintaining the inference performance consistent. Furthermore, our approach adds minimal overhead to the cost incurred (wall clock time) at training time. The proposed approach shows strong performance on a wide variety of datasets and models, even outperforming strong baselines such as distilled ensembles as well as combinatorial optimization methods based on submodular optimization.

==> old_abstract.tex <==
Recent breakthroughs and successful deployment of large language and vision models predominantly follow a two phase approach. First, large models are trained to achieve recordbreaking results, followed by compression/quantization for deployment in memory limited applications, or the use of knowledge distillation for low latency tasks. Formally, this can be seen as the problem of identifying an optimal model of size n from a larger model of size $k \cdot n$, where $k > 1$ is the overparameterization factor. In this paper, we ask if can develop a single training run that can simultaneously train a larger model and derive a smaller model for deployment? In order to do this, we propose and investigate {\it simulated overparameterization}: a new way to train large models that can be directly converted to a smaller model at inference time. 
 
%Recent breakthroughs in large language and vision models would not be possible without model scaling. However, at deployment time larger models often undergo a secondary {\it downsizing} phase. This phase usually takes the form of model compression and quantization for applications where memory is a limiting factor, or model distillation for applications where inference latency is the bottleneck. Denoting the number of parameters $n$ as a proxy for model size, the overall model deployment process can then be viewed as finding the best model of size $n$ via leveraging the capabilities of a larger size $k \cdot n$ model, where $k > 1$ is an overparameterization factor. In this work, we ask if a single training run be used to simultaneously perform training and obtain a smaller model, that can be deployed at inference time? In order to do this, we propose and investigate {\it simulated overparameterization}: a new way to train large models that can be directly converted to a smaller model at inference time. 

We propose a simple yet effective architectural change namely, {\em Majority Kernels} that are compatible with many standard architectures such as multi-layer perceptrons (MLPs), Residual networks (ResNets), and Transformers. We demonstrate that via majority kernels we can perform simulated training of overparameterized models resulting in performance gains across architectures and tasks. Furthermore, our approach adds minimal overhead to the cost incurred (wall clock time) at training time. The proposed approach shows strong performance on a wide variety of datasets and models, even outperforming strong baselines such as combinatorial optimization methods based on submodular optimization. 

%Recent breakthroughs and successful deployment of large language and vision models predominantly follow a two phase approach. First, large models are trained to achieve recordbreaking results, followed by compression/quantization for deployment in applications that are constrained by small memory footprint, or the use of knowledge distillation for low latency serving tasks. Formally, we can jointly look at this problem as searching for an optimal model of size n from a much larger model of size kn, where k>1 is the overparameterization factor. In this paper, we ask if can combine the two phases and develop a single training run that simultaneously trains a larger model and still find an optimal smaller model for deployment? In order to do this, we propose and investigate {\it simulated overparameterization}: a new way to train large models that can be directly converted to a smaller model at inference time. 


%We also propose an alternate, more computationally intensive approach via modeling the problem of selecting the best $k$ parameters out of $k \cdot n$ parameters as that of solving multiple submodular optimization problems. We demonstrate the efficacy of our proposed approach on real data and discuss challenges in scaling it for larger models.

% Model scaling is one of the key contributors in the astonishing performance of deep learning over the past decade. However, at deployment time large models often undergo a secondary {\it downsizing} phase. This phase usually takes the form of model compression and quantization for applications where memory is a limiting factor, or model distillation for applications where inference latency may be a concern. Denoting the number of parameters $n$ as a proxy for model size, the overall model deployment process can then be viewed as finding the best size $n$ model via leveraging the capabilities of a larger size $k \cdot n$ model, where $k > 1$ is an overparameterization factor. In this work we study whether the above goal can be achieved entirely within a single training run itself. We propose and study {\it simulated overparameterization}: a way to train large models that can be directly converted to a smaller model at inference time. 

% We propose a simple yet effective architectural change namely, {\em majority kernels} that are compatible with many standard architectures such as multi-layer perceptrons (MLPs), Residual networks (ResNets), and Transformers. We demonstrate that via majority kernels it is indeed possible to perform simulated training of overparameterized models resulting in performance gains across architectures and tasks. Furthermore, our approach adds minimal overhead to the cost incurred (wall clock time) at training time. 

% We also propose an alternate, more computationally intensive approach via modeling the problem of selecting the best $k$ parameters out of $k \cdot n$ parameters as that of solving multiple submodular optimization problems. We demonstrate the efficacy of our proposed approach on real data and discuss challenges in scaling it for larger models.

% TODO:\pranjal{I just picked an arbitrary author order. Hanna should be first author. Others can be randomized by coin toss.}

==> old_bae.tex <==
% In this subsection, we analyze the implicit gradient regularization terms that are introduced from training with our algorithm. 

% % Let $L_o: \mathbb{R}^n \rightarrow \mathbb{R}$ be the original loss function of the original optimization before expanding the parameters. Let $L_e: \mathbb{R}^{n\times e}\rightarrow \mathbb{R}$ be the evaluation loss of our algorithm, and $L_t: \mathbb{R}^{n\times e}\rightarrow \mathbb{R}$ be the training loss function. Here note that our expansion scale is $e$. We have,
% % $$
% % L_e(\gamma_{11}, \gamma_{12}, \ldots, \gamma_{1e}, \gamma_{21}, \ldots, \gamma_{ne}) = L_o\left(\frac{\gamma_{11} + \gamma_{12} + \cdots + \gamma_{1e}}{e}, \ldots, \frac{\gamma_{n1} + \gamma_{n2} + \cdots + \gamma_{ne}}{e} \right),
% % $$
% % and,
% % $$
% % L_t(\gamma_{11}, \gamma_{12}, \ldots, \gamma_{1e}, \gamma_{21}, \ldots, \gamma_{ne}) = L_o\left(p_{11}\gamma_{11} + \cdots + p_{1e}\gamma_{1e}, \ldots, p_{n1}\gamma_{n1} + \cdots + p_{ne}\gamma_{ne} \right),
% % $$
% % for random $p_{ij}\in \mathbb{R}$, where $\sum_j p_{ij}=1$ for all $i\in[n]$.
% Recent work \citep{barrett2020implicit} uses Backward Error Analysis (BEA) has shown that for any sufficiently differentiable loss function~($L$), gradient decent follows a modified loss surface ($\tilde{L}$) when training defined as:
% %
% \begin{equation}\label{gradient_reg_term}
% \tilde{L}(w) = L(w) + \frac{\ell}{4} \lVert \nabla_w L(w) \rVert_2^2
% % L(w) + \frac{\ell}{4} \sum_{\theta_i}\left(\nabla_{\theta_i} L(\theta)\right)^2
% \end{equation}
% %
% where $\ell \in \mathbb{R}$ is the learning rate. The extra term acts as a regularization term and favors parameters points with low gradient which might mean flatter minima.

% To analyze our algorithm recall that in our algorithm, given any parameter $\theta_i$ we replace it with $e$ parameters $(\gamma_{i1}, \ldots, \gamma_{ie})$, and the final model parameters $\theta_i$ will get the mean of $(\gamma_{i1}, \ldots, \gamma_{ie})$. 
% % That is,
% % $$
% % \theta_i = g(\gamma_{i1}, \ldots, \gamma_{ie}) = \frac{(\gamma_{i1}, \ldots, \gamma_{ie})}{e}
% % $$
% % If we were to perform gradient descent on the evaluation loss $L_e$, then we have that
% % % the loss function can be written in the following way,
% % % $$
% % % L(\ldots, \theta_i, \ldots) = L(\ldots, g(\gamma_1, \ldots, \gamma_e),\ldots)
% % % $$
% % % and thus, we will end having the following gradients for $\gamma_j$
% % \begin{align}
% % \nabla_{\gamma_{ij}} L_e(\gamma) &= \nabla_{\gamma_{ij}} L_o(\ldots, \frac{\gamma_{i1} + \cdots + \gamma_{ie}}{e}, \ldots)  \nonumber \\ &= \nabla_{\theta_i} L_o(\ldots, \theta_i, \ldots) \nabla_{\gamma_{ij}} \frac{\gamma_{i1} + \cdots + \gamma_{ie}}{e} = \frac{\nabla_{\theta_i} L}{e}.\label{mean_gradient}
% % \end{align}
% % \begin{lemma}
% % Performing a gradient descent step with learning rate $\ell$ on the loss $L_e$ where each $\theta_i$ is a mean of $e$ variables is equivalent to performing a gradient descent step on original $L_o$ with learning rate $\ell/e$.
% % \end{lemma}
% % \begin{proof}
% % when performing gradient descent with learning rate $\ell/e$ on the original loss we have 
% % $$
% % \theta_i \gets \theta_i - \frac{\ell}{e} \nabla_{\theta_i} L_o(\theta),
% % $$
% % and from (\ref{mean_gradient}), we know that each $\gamma_{ij}$ is updated as follows when performing a gradient descent step with learning rate $\ell$
% % $$
% % \gamma_{ij} \gets \gamma_{ij} - \frac{\ell}{e} \nabla_{\theta_i} L(\theta).
% % $$
% % The proof follows immediately from the fact that moving all elements in a vector by $\frac{\ell}{e} \nabla_{\theta_i}$ moves the average of that vector by $\frac{\ell}{e} \nabla_{\theta_i}$.
% % \end{proof}
% % Note that the gradient regularization term  (\ref{gradient_reg_term}) in the loss surface $L_e$ when descending with learning rate~$\ell$ is equivalent to the gradient regularization term on the original problem $L_o$ when training with learning rate~$\ell/e$. To see this note that from~(\ref{mean_gradient}) we have,
% % $$
% % \frac{\ell}{4} \sum_{\gamma_{ij}}\left(\nabla_{\gamma_{ij}} L(\gamma)\right)^2 = \frac{\ell}{4} \sum_{\theta_i}e\left(\frac{\nabla_{\theta_i} L(\gamma)}{e}\right)^2 =   \frac{\ell}{4e} \sum_{\theta_i}\left(\nabla_{\theta_i} L(\theta)\right)^2.
% % $$
% % Now after showing that expanding a parameter to be an average of $e$ shadow parameters does not change our optimization (that is, gradient descent on $L_e$ is equivalent to $L_o$), we will prove that by training on $L_t$ instead our algorithm increases the implicit gradient regularization compared to vanilla training.
% %%%%%%%%%%%%%%%%%%%%% NEW %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We start by applying backward error analysis to understand the modified loss surface we follow in our algorithm. We will conduct our analysis on the simulated over-parameterized space/surface $\mathbb{R}^{n\times e}$ first and then make a switch to the collapsed original model loss space $\mathbb{R}^n$ in order to be able to compare with vanilla training (i.e., we start with the space of $\gamma$ and then switch to~$\theta$). 
% In the simulated over parameterization space $\mathbb{R}^{n\times e}$, we can compare our algorithm implicit gradient regularization with that of the same algorithm on the same space but with equal probabilities, and using Lemma~\ref{uniform_fallback} we can conclude how our implicit gradient regularization behave compared to the original problem on the original space $\mathbb{R}^n$ (Corollary~\ref{higher_implicit_reg}).

% Our analysis is similar to \citep{barrett2020implicit}, where we view gradient decent as explicit Euler method numerically integrating the vector field~$f(\gamma)=-\nabla_\gamma L(\gamma, p)$ where $p\in\mathbb{R}^{n\times e}$ is the selected probabilities vector for the batch.

% We define
% $$
% \tilde{f}(\gamma) = f_e(\gamma) +\ell^0 f_0(\gamma) + \ell f_1(\gamma) + \ell^2 f_2(\gamma) + \cdots,
% $$
% to be modified vector field with correcting terms in powers of the step size and $f_e =-\nabla_\gamma L(\gamma, (1/e)^{n\times e})$.
% %(correcting from $f_e = -\nabla_\gamma L_e(\gamma)$ rather than $f_t$). 
% We show the following,

% \begin{restatable}[Backward Error Analysis]{theorem}{bea}
% \label{th:bea}
% Let $L_o$ be a sufficiently differentiable function on a parameter space $\theta\in \mathbb{R}^n$. The modified equation for gradient flow when using Majority Kernels is of the form
% $$
% L_o(\theta) + c\frac{\ell}{4e} ||\nabla_\theta L_o(\theta)||^2 + \frac{1}{e} \left<\epsilon, \nabla_\theta L(\theta)\right> + O(\ell^2 + ||\epsilon||^2).
% $$
% where $c \in \mathbb{R}$ is greater than one, $\epsilon \in \mathbb{R}^n$ is the perturbation measuring the difference between the training chosen parameters and the evaluation ones (in the original nonover-parameterized space. Here the expected value of $\epsilon$ is $E(\epsilon) = 0^n$, see previous Section for more details). 
% \end{restatable}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{theorem}
% Let $L$ be a loss function. When applying the majority kernel algorithm, the implicit gradient regularization term with learning rate $\ell$ is greater or equal to the implicit regularization term of the original loss with learning rate $\ell /e$.
% \end{theorem}
% \begin{proof}
% When applying a train step in the majority kernel algorithm, given a parameters $\theta_i$, we apply 
% $$
% \theta_i \gets p_1 \gamma_1 + \cdots + p_e \gamma_e,
% $$
% where $p_1+\cdots+p_e = 1$. Similar to equation (\ref{mean_gradient}), we have
% \begin{equation}\label{majority_gradient}
% \nabla_{\gamma_j} L(\ldots, (p_1\gamma_1 + \cdots + p_e \gamma_e), \ldots) = p_j\nabla_{\theta_i} L.
% \end{equation}
% The above suggest that the gradient $\nabla_{\theta_i} L$ is split and applied to the parameters $\gamma_j$ based on their randomly drawn probability $p_j$. Now, if we try to calculate the implicit gradient regularization term from (\ref{gradient_reg_term}) we get
% $$
% \frac{\ell}{4} \sum_{\gamma_i}\left(\nabla_{\gamma_i} L(\gamma)\right)^2 = \frac{\ell}{4} \sum_{\theta_i} \left((p_1^2 + \cdots + p_e^2) \cdot (\nabla_{\theta_i} L(\theta))^2  \right) \geq \frac{\ell}{4e} \sum_{\theta_i} (\nabla_{\theta_i} L(\theta))^2.
% $$
% The inequality above follows from the fact that $p_1 + \cdots + p_e = 1$ and that $p_j \geq 0$ for all $j$; If we apply Cauchy–Schwarz inequality: $|\left<u,v\right>|^2 \leq \left<u, u\right> \left<v, v\right>$, where we set $u = (p_1, \ldots, p_e)$ and $v = (1,\ldots, 1)$, we get 
% $$
% \left(\sum_i p_i\right)^2 = 1^2 \leq (1+\cdots+1) (p_1^2 + \cdots + p_e^2) = e (p_1^2 + \cdots + p_e^2), 
% $$
% Thus, $(p_1^2 + \cdots + p_e^2) \geq 1/e$, which concludes the proof.
% \end{proof}

%\input{subset}

==> old_intro.tex <==
\section{Introduction}
\label{sec:intro}

Unlocking the true potential of deep learning architectures trained via first order methods often requires training models that have large sizes, as measured by the number of parameters. We are witnessing a consistent and monotonic increase of performance with the model size with no signs of diminishing gains or saturation. Larger model training is inevitable, and we have been witnessing this from the early groundbreaking computer vision results with CNNs~\citep{krizhevsky2012imagenet,szegedy2015going} and ResNets~\citep{he2016deep} to all encompassing transformer architectures~\citep{vaswani2017attention, brown2020language, chowdhery2022palm, chen2022pali} on language modeling and beyond.

\newtext{Historically, to achieve state-of-the-art performance, researchers modified both architectures and training algorithms as they scaled models [CITES..]. This implicitly favored architectures that excelled with larger parameter counts. However, a growing awareness of compute-to-performance curves has shifted attention toward sparse architectures with high-capacity backbones [CITE..]. These architectures might not achieve the absolute best results per parameter, but their superior compute scalability leads to a significantly improved compute-to-performance ratio.}

%Starting from the groundbreaking work of \citet{krizhevsky2012imagenet}, large CNN based models such as the Inception architecture \citep{szegedy2015going} and Residual Networks \citep{he2016deep} achieved state-of-the-art performance for many problems in computer vision. In recent years, a similar trend has been observed in language modeling where larger and larger transformer models \citep{vaswani2017attention} continue to display surprising general purpose capabilities \citep{brown2020language, chowdhery2022palm, chen2022pali}.


\deletetext{However,} \newtext{While sparse architectures excelled reducing training compute,} when it comes to deploying large models \newtext{however} one has to meet strict real world constraints. Models on smartphones need to operate in the presence of strict memory constraints. Similarly, models processing billions of queries in real time have to minimize the inference latency. Such considerations have led do a large body of work where a large model is first trained and then post-processed to fit the desired criteria. For instance techniques in model pruning and quantization aim to produce models with reduced memory requirements \citep{lecun1989optimal, han2015deep, frankle2018lottery, cai2020zeroq, nagel2020up}. Similarly, the aim of model distillation is to train smaller models that can faithfully approximate a larger model (typically of the same architecture) \citep{Hinton06, buci2006model}. 

Hence the overall process of training and deploying ML models in the real world is often decomposed into two phases: an initial phase where a larger model is trained, and a secondary phase where the model is downsized to accommodate the application at hand. In this work we ask the following intriguing question: can a single training run be used to simultaneously perform a large scale training and obtain a smaller model that is ready to use off-the-shelf at inference time? \newtext{I.e., can we overparameterize a small backbone model in a way that introduce small overhead in training, and falls back on the original small model in inference?} We call this training paradigm as {\it simulated overparameterization} as it involves implicitly training a much larger model than the one for intended use case.

We propose a simple approach towards achieving the goal of simulated overparameterization. Our approach namely {\it majority kernels} is an effective method that can be applied to a variety of architectures. To describe the core idea behind majority kernels consider a model \( M: {\cal X} \rightarrow \mathbb{R}^k \), where \( {\cal X} \subseteq \mathbb{R}^d \) represents the domain of the data distribution. Define \( M \) as an ensemble of \( e \) different models: \( M(x) = \frac{1}{e} \sum_{i=1}^e M_i(x) \) for \( x \in {\cal X} \). It is well understood that ensembling of models often produces a model that is superior and more robust as compared to the base models \citep{huang2017snapshot, fort1912deep}. Although typically ensembling is done in the model (function) space, if one could do ensembling in the parameter space itself then $M$ would correspond to a powerful model that is also small in size. However, naive ensembling in the parameter space often performs poorly as the parameters of the different models might not be aligned along the same local optima. \textcolor{blue}{Sri: This somewhat makes sense. To clarify this further, it would also be good to add another statement explaining why this misalignment would cause challenges in achieving the best ensembled model.}
%
% In order to force the right alignment, we directly incorporate the $k$ different model parameters into a single training process. Specifically, within each iteration of mini batch gradient descent we perform a forward pass via a network that uses a random linear combination of the model parameters and perform backpropagation to update  all the $k$ different parameters. Finally, at inference time we simply perform uniform averaging in the parameter space to compute the final model. Across a variety of architectures and datasets we demonstrate that majority kernels are an effective technique for implicitly performing overparameterized training.

In order to force the right alignment, we simulate the overparameterization of each layer incorporating the parameters of $e$ extra models integrated into a single training process.
%
Specifically, within each iteration of mini batch gradient descent we perform a forward pass with a set of virtual parameters, $\theta \in \mathbb{R}^n$. These are the result of applying function $s_p: \mathbb{R}^{n \times e} \times \mathbb{R}^{n \times e} \to \mathbb{R}^n$, a random linear combination of the overparameterized model parameters, $\tilde{\theta} \in \mathbb{R}^{n\times e}$. We then perform backpropagation to update all the $e$ different parameters.
%
Finally, at inference time we simply perform uniform averaging in the parameter space to compute the final model ($s: \mathbb{R}^{n \times e} \to \mathbb{R}^n$).
%
We call this process ``simulated'' because the forward pass of the network is performed on $\mathbb{R}^n$ by aggregating the extra parameters stochastically.

In our study, we explore the efficacy of majority kernels across different architectures and datasets, showcasing their role in facilitating implicit overparameterized training.
%
Additionally, we analyze the algorithm through the lenses of implicit regularization and sharpness-aware minimization. This approach helps us understand how the algorithm not only naturally limits the complexity of the models but also seeks out more stable and generalizable solutions by focusing on flatter areas in the loss landscape. This analysis provides clearer insights into how and why the algorithm performs effectively.

In summary, Simultaneous Overparameterization (SOP) aims to balance the computational efficiency of smaller models with the enhanced learning capabilities of larger, overparameterized models. SOP is characterized by its unique approach to model training and inference, where a model with a significantly larger number of parameters is trained in such a way that a smaller, efficient subset of these parameters is used for the actual computation during inference. This paradigm allows for the benefits of overparameterization, such as improved training dynamics and generalization, while maintaining computational efficiency.

\iffalse
The second approach namely {\it subset selection} is based on submodular optimization \citep{fujishige2005submodular, krause2014submodular}. Consider a one layer MLP $M(x) = v^T \sigma(W \cdot x)$, where $x \in \mathbb{R}^d$, $W \in \mathbb{R}^{m \times d}, v \in \mathbb{R}^m$ and $\sigma$ is the ReLU activation. Given an overparameterization factor of $k > 1$, we maintain at each step $t$, model parameters $\{v_t, U_t\}$ where $U_t \in \mathbb{R}^{k \cdot m, d}$. Additionally, before each mini batch gradient step we select $m$ out of the $k \cdot m$ rows in $U_t$ to perform the forward and the backward passes. We model the problem of selecting the best $m$ rows as that of optimizing a submodular objective that balances utility of the neurons (rows) and their diversity. The final network that is inference ready is obtained by selecting the best $m$ rows of the $U_t$ matrix at the end of training. We demonstrate the effectiveness of the approach on both vision and language tasks. However the approach of subset selection is computationally more expensive thereby preventing us from experimenting with very large models. We discuss challenges and future directions related to this towards the end of the paper.
\fi



==> old_mk_intro.tex <==
Simulated overparameterization is a concept that involves using more nodes in a network than it typically contains, without increasing computational complexity. One method to achieve this is through Majority Kernels (MK). This approach involves training each layer of a Deep Neural Network (DNN) with an expanded version of their internal kernels. During training, MK synthesizes these expanded kernels by randomly averaging extra parameters into the layer's original dimensions. At the inference stage, the kernel reverts to the average of these expanded versions.

The benefits of this method include:
\begin{itemize}
  \item Maintaining manageable computational complexity during the training phase.
  \item Enabling automatic distillation of the inference parameters of the model.
  \item Enhancing parameter weight optimization, which helps avoid local minima by smoothing the loss landscape during training.
\end{itemize}

This section will describe the algorithm and its inherent optimization effects by discussing the implicit gradient regularization achieved through backward error analysis and how this method proves more efficient than standard Stochastic Gradient Descent (SGD). Also, we will analyze its stochastic sharpness-aware minimization effect.

==> old_sam.tex <==
\subsection{A Sharpness Aware Minimization with Variable Implicit Gradient Regularization}\label{sec:majority_theory}

This section delves into the theoretical underpinnings of our algorithm, focusing on two key aspects. First, we demonstrate that our algorithm essentially implements sharpness-aware minimization. It achieves this by minimizing the average loss within an $\epsilon$-neighborhood, where $\epsilon$ dynamically changes throughout training. Second, we show that our algorithm produces implicit gradient regularization that is higher than vanilla training with SGD with an appropriate learning rate (see Lemma~\ref{uniform_fallback} and Corollary~\ref{higher_implicit_reg}). Importantly, this implicit regularization is variable and fluctuates randomly with each batch, ensuring it never falls below the level of vanilla SGD.

% In this section, we theoretically analyze two aspects of our algorithm. We show that our algorithm act as a sharpness aware minimization where it minimizes the loss for an $\epsilon$ neighborhood where $\epsilon$ is based on the learning; Addition throughout training, our algorithm produces implicit gradient regularization that is higher than vanilla training with SGD with appropriate learning rate (see Lemma \ref{} and Corollary \ref{}). The implicit gradient regularization is variable and fluctuate randomly in every batch without going below the implicit gradient regularization of vanilla sgd training.

Before diving into the two aspects, we first show a simple lemma showing that if the probabilities are equal throughout training then our algorithm falls back on SGD with smaller learning rate.

\begin{lemma}\label{uniform_fallback}
When the probabilities in the probability tensors $P_r$ in the algorithm are equal (uniform), then our gradient decent step with learning rate $\ell$ is equivalent to a gradient decent step on the original problem without expansion with learning rate $\nicefrac{\ell}{e}$.
\end{lemma}
\begin{proof}
In our algorithm, given any parameter $\theta_i$ we replace it with $e$ parameters $(\gamma_{i1}, \ldots, \gamma_{ie})$, where for the final model parameters $\theta_i$ will get the mean of $(\gamma_{i1}, \ldots, \gamma_{ie})$. 

Now, when performing gradient descent with learning rate $\nicefrac{\ell}{e}$ on the original loss we have 
$$
\theta_i \gets \theta_i - \frac{\ell}{e} \nabla_{\theta_i} L(\theta).
$$
If we were to perform gradient descent in our algorithm with equal probabilities $(1/e)$, then we have that
\begin{align}
\nabla_{\gamma_{ij}} L_{ours}(\gamma) &= \nabla_{\gamma_{ij}} L(\ldots, \frac{\gamma_{i1} + \cdots + \gamma_{ie}}{e}, \ldots)  \nonumber \\ &= \nabla_{\theta_i} L(\ldots, \theta_i, \ldots) \nabla_{\gamma_{ij}} \frac{\gamma_{i1} + \cdots + \gamma_{ie}}{e} = \frac{\nabla_{\theta_i} L}{e}.\label{mean_gradient}
\end{align}

Thus, when performing gradient descent with our algorithm with learning rate $\ell$ with equal probabilities, each $\gamma_{ij}$ is updated as follows
$$
\gamma_{ij} \gets \gamma_{ij} - \frac{\ell}{e} \nabla_{\theta_i} L(\theta).
$$
The proof follows immediately from the fact that moving all elements in a vector by $\frac{\ell}{e} \nabla_{\theta_i}$ moves the average of that vector by $\frac{\ell}{e} \nabla_{\theta_i}$.

\end{proof}
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.5]{majority_kernel_theory_overview.pdf}
    \caption{Overview of the algorithm's dynamics.}
    \label{fig:majority_theory_overview}
\end{figure}

Now, after understanding the importance of the random probabilities, we analyze our algorithm for random probabilities. We start with sharpness aware minimization.

\subsubsection{Sharpness Aware Minimization}
Sharpness-Aware Minimization (SAM) aims to find parameters that not only minimize the training loss,
$L(\theta)$, but also maintain a low loss in the vicinity of $\theta$, thereby leading to solutions that generalize better.
SAM achieves this by considering both $L(\theta)$ and $L(\theta + \epsilon)$, where $\epsilon$ is a perturbation that maximizes the
loss within a defined neighborhood of $\theta$.

In our algorithm, the perturbation happens naturally via our stochastic approach. Recall that in our algorithm each variable is expanded to be a mean of $e$ ones. That is,
$$
\theta_i = \frac{1}{e} \sum_{j=1}^e \gamma_{ij}.
$$
When applying random probabilities $p_{ij}$ instead of $\nicefrac{1}{e}$, we get
$$
\theta_i' =  \sum_{j=1}^e p_{ij} \gamma_{ij} = \sum_{j=1}^e ((p_{ij} - \frac{1}{e}) \gamma_{ij} + \frac{1}{e} \gamma_{ij}) = \theta_i + \sum_{j=1}^e (p_{ij} - \frac{1}{e})\gamma_{ij}
$$
Thus, our perturbation in each step is random
$$
\epsilon_i = \sum_{j=1}^e (p_{ij} - \frac{1}{e})\gamma_{ij}.
$$
It is easy to see that the mean of our perturbation is zero
$$
E[\epsilon_i] = E\left[\sum_{j=1}^e (p_{ij} - \frac{1}{e})\gamma_{ij}\right] = \sum_{j=1}^e E\left[(p_{ij} - \frac{1}{e})\gamma_{ij}\right] = \sum_{j=1}^e \gamma_{ij} E\left[(p_{ij} - \frac{1}{e})\right] = 0.
$$
The variance of our perturbation is
$$
E[\epsilon_i^2] = E\left[\left(\sum_{j=1}^e (p_{ij} - \frac{1}{e})\gamma_{ij}\right)^2\right] = E\left[\left(\sum_{j=1}^e p_{ij}\gamma_{ij} - \theta_i \right)^2\right].
$$
Note the following, since $\sum_{j=1}^e p_{ij} = 1$, then it is easy to see that if all $\gamma_{ij}$ are equal (in such case, they must be equal to $\theta_i$ since $\theta_i = \sum_{j=1}^e \frac{1}{e} \gamma_{ij}$), then our variance is zero, that is, $E[\epsilon_i^2]=0$. In such case, our descent is not sharpness aware. However, our variance grows the more inconsistency exists between the~$\gamma_{ij}$'s; meaning, the more these shadow variables disagree, the algorithm is biased to descent to loss points with larger neighborhood with expected loss that is small.

In the next subsection, we show that even if the shadow variable agree, our implicit gradient regularization is guaranteed to be higher than regular gradient descent and thus possibly converge to a flatter minima (Corollary~\ref{higher_implicit_reg}).

==> sop.tex <==
\section{The Simulated Overparameterization Paradigm}

In this section we describe in detail the paradigm of Simulated Overparameterization (SOP).
% In this work, we introduce the concept of Simulated Overparameterization (SOP), a novel paradigm in machine learning that combines the computational efficiency of small models with the superior learning capabilities of larger, overparameterized models. 
SOP involves training a model with a significantly larger number of parameters in such a way that a smaller, efficient subset of these parameters is used for the actual computation during inference. This method offers the advantages of overparameterization, such as improved training and generalization, while keeping computational demands low.

The SOP paradigm is built upon the following key principles:

\begin{enumerate}[leftmargin=*]
    \item \textbf{Extended Training Dynamics}: SOP aims to balance computational efficiency with enhanced learning performance, leveraging a larger total parameter set for training while using a smaller set for inference.
    \item\textbf{Limited Training Overhead}: SOP assumes an increase in the amount of model parameters we are able to train given a small cost of compute per step. Hence, training compute is within the same order of magnitude with just a small overhead. $T \approx \mathcal{O}(B) + \gamma$, where $T$ represents the train compute, $B$ represents the base compute, and $\gamma \ll B$ symbolizes a small overhead.
    \item\textbf{Dual-Parameter Utilization}: The number of parameters used during the forward pass and inference is the same so it avoids a second step to post-process the model.
    \item\textbf{Adaptive Parameter Management}: Dynamic selection of parameters is employed, balancing smaller model efficiency and larger model capacity.
\end{enumerate}

Assuming \( e \) as the overparameterization factor, we formalize the two classes of models within the SOP paradigm in definitions~\ref{def:model_o} and \ref{def:model_e}.

\begin{restatable}[Overparameterized Model Class]{definition}{ModelO}
\label{def:model_o}
The Overparameterized Model Class, \( \mathcal{M}_O \), with a parameter set \( \thetae \in \mathbb{R}^{n \times e} \), represents a higher-dimensional space of the model's parameters.
%
\( \mathcal{M}_O \) is utilized during the training phase to exploit the advantages of a larger parameter set.
%
Although \( \mathcal{M}_O \) receives gradient updates across its entire parameter set during forward computations, an aggregation function \( s \) is applied to a subset of \( \thetae \) to form the virtual parameters used in \( \mathcal{M}_E \).
\end{restatable}

\begin{restatable}[Efficient Model Class]{definition}{ModelE}
\label{def:model_e}
The Efficient Model Class, \( \mathcal{M}_E \), operates with a virtually simulated parameter set \( \theta \in \mathbb{R}^n \). These parameters are an aggregated version of \( \thetae \) and are not physically instantiated. \( \mathcal{M}_E \) is employed for efficient computation during both training and inference, simulating a smaller, computationally tractable model.
\end{restatable}

Within the SOP framework, each iteration of mini-batch gradient descent involves a forward pass using the set of virtual parameters, \( \theta \). These virtual parameters are the result of applying a function \( s_p: \mathbb{R}^{n \times e} \to \mathbb{R}^n \) on the overparameterized model's parameters, \( \thetae \). This process defines the Efficient Model Class with the virtually aggregated parameters used for computation.
%
Subsequently, backpropagation is performed to update all the \( n \times e \) different parameters in~\( \thetae \). This update process ensures that the learning benefits of~\( \thetae \) are fully realized, while the computational efficiency is maintained through the use of the virtual parameter set~\( \theta \).
%
Finally, at inference time we simply perform uniform averaging in the parameter space to compute the final model by applying function $s: \mathbb{R}^{n \times e} \to \mathbb{R}^n$.

Several algorithms can potentially align with SOP principles. These can be broadly categorized into three types: (1) \textbf{Stochastic}, which randomly combines extra kernels; (2)~\textbf{Adaptive}, learning the interdependency of extra parameters; and (3) \textbf{Elimination}, ranking and retaining only the important kernels. Our work introduces a unique approach within the Stochastic category, adhering to SOP's core principles. The details are discussed in the following sections.

